Direct shape optimization through deep reinforcement learning

Deep Reinforcement Learning (DRL) has recently spread into a range of domains within physics and engineering, with multiple remarkable achievements. Still, much remains to be explored before the capabilities of these methods are well understood. In this paper, we present the first application of DRL to direct shape optimization. We show that, given adequate reward, an artificial neural network trained through DRL is able to generate optimal shapes on its own, without any prior knowledge and in a constrained time. While we choose here to apply this methodology to aerodynamics, the optimization process itself is agnostic to details of the use case, and thus our work paves the way to new generic shape optimization strategies both in fluid mechanics, and more generally in any domain where a relevant reward function can be defined.

==> fig/3pts_area.tex <==
\begin{figure}
\centering

\setlength{\fboxsep}{0pt}%
\setlength{\fboxrule}{1pt}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[t]{.25\textwidth}
	\centering
	\fbox{\includegraphics[width=\linewidth]{fig/4_pts_3_pts_area.png}} 
	\caption{Best shape with 4 points, 3 free points, with area penalization ($\alpha = 3.176$)}
	\label{fig:4_pts_3_pts_area}
\end{subfigure} \qquad \qquad
\begin{subfigure}[t]{.25\textwidth}
	\centering
	\fbox{\includegraphics[width=\linewidth]{fig/4_pts_3_pts.png}} 
	\caption{Best shape with 4 points, 3 free points, no area penalization ($\alpha = 2.733$)}
	\label{fig:4_pts_3_pts_no_area}
\end{subfigure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{\textbf{Optimal shapes obtained with and without area penalization} using 4 points with 3 free points. While the target area is that of the unit cylinder ($\alpha_{\text{cyl}} = \pi$), the area of the optimal shape with area penalization is equal to 3.176, versus 2.733 for that of the non-penalized shape. While respecting this constraint, the lift-to-drag ratio of the penalized shape is approximately 30\% lower than that of the non-penalized one.}
\label{fig:3pts_area}
\end{figure} 

==> fig/4_pts_leading_edge.tex <==
\begin{figure}
\centering

\setlength{\fboxsep}{0pt}%
\setlength{\fboxrule}{1pt}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[t]{.25\textwidth}
	\centering
	\fbox{\includegraphics[width=\linewidth]{fig/4_pts_4_pts.png}} 
	\caption{Best shape with 4 free points}
\end{subfigure} \qquad
\begin{subfigure}[t]{.25\textwidth}
	\centering
	\fbox{\includegraphics[width=\linewidth]{fig/4_pts_4_pts_leading_edge.png}} 
	\caption{Close-to-best shape with 4 free points}
\end{subfigure} \qquad
\begin{subfigure}[t]{.25\textwidth}
	\centering
	\fbox{\includegraphics[width=\linewidth]{fig/4_pts_4_pts_leading_edge_2.png}} 
	\caption{Close-to-best shape with 4 free points}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{\textbf{Some of the best performers using 4 free points.} A rounded leading edge is not an essential feature of the best performers. This arises from the low $Re$ value used in this experiment. By contrast, the trailing edge is similar in all the best-performing shapes.}
\label{fig:4_pts_leading_edge}
\end{figure} 

==> fig/DRL.tex <==
\begin{figure}
\centering
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\myscale{1.0}
\begin{tikzpicture}[	scale=\myscale,
				arrow/.style={thick,color=mybluegray3,rounded corners}]

	%%%%% nodes
	\node[	scale=\myscale,
			rectangle, rounded corners, draw=mygray1, fill=mygray4, thick, 
			text width=2cm, minimum height=1cm, text centered,
			inner sep=2pt, outer sep=0pt] 
			(env) at (0,0) {\footnotesize Environment};
	\node[	scale=\myscale,
			rectangle, rounded corners, draw=myorange1, fill=myorange4, thick, 
			text width=2cm, minimum height=1cm, text centered,
			inner sep=2pt, outer sep=0pt] 
			(agent) at (5,0) {\footnotesize Agent};
	
	%%%%% arrows
	\draw[-stealth,arrow] (env.east) -- (agent.west);
	\draw[-stealth,arrow] (agent.south) to [out=-90,in=-90] (env.south);
	\draw[-stealth,arrow] (env.north) to [out=90,in=90] (agent.north);

	%%%%% arrow writings
	\draw[draw=none,postaction={decorate,decoration={raise=0.5ex,text along path,text align=center,text={|\footnotesize|Reward}}}] (env.east) -- (agent.west);
	\draw[draw=none,postaction={decorate,decoration={raise=-1.5ex,text along path,text align=center,text={|\footnotesize|Actions}}}] (env.south) to [out=-90,in=-90] (agent.south);
	\draw[draw=none,postaction={decorate,decoration={raise=0.5ex,text along path,text align=center,text={|\footnotesize|Observations}}}] (env.north) to [out=90,in=90] (agent.north);

\end{tikzpicture}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{\textbf{General reinforcement learning framework}. }
\label{fig:DRL}
\end{figure} 

==> fig/boat_tailing_4pts.tex <==
\begin{figure}
\centering

\setlength{\fboxsep}{0pt}%
\setlength{\fboxrule}{1pt}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[t]{.25\textwidth}
	\centering
	\fbox{\includegraphics[width=\linewidth]{fig/4_pts_4_pts_boat_tailing.png}} 
	\caption{Best shape with forced symmetry (7 d.o.f.s)}
	\label{fig:4_pts_sym}
\end{subfigure} \qquad
\begin{subfigure}[t]{.25\textwidth}
	\centering
	\fbox{\includegraphics[width=\linewidth]{fig/4_pts_4_pts_boat_tailing.png}} 
	\caption{Best shape without forced symmetry (12 d.o.f.s)}
	\label{fig:4_pts_free}
\end{subfigure}

\bigskip

\begin{subfigure}[t]{.4\textwidth}
	\centering
	\begin{tikzpicture}[scale=0.875,trim axis left, trim axis right]
		\begin{axis}[	xlabel=episodes, ylabel=reward,
					grid=major,xmin=0,xmax=4000,ymin=-2,ymax=2,legend cell align=left,
            				every axis y label/.style={at={(ticklabel cs:0.5)},rotate=90,anchor=near ticklabel}]
			\legend{$\left<r_t\right>$ with symmetry, $\left<r_t\right>$ w/o symmetry}
 
			\addplot[draw=myblue1,thick,smooth] 		table[x index=0,y index=2] {fig/reward_4_pts_4_pts_boat_tailing}; 
			\addplot[draw=myorange1,ultra thick,smooth] 	table[x index=0,y index=2] {fig/reward_4_pts_4_pts_boat_tailing}; 
		\end{axis}
	\end{tikzpicture}	
	\caption{Moving-average reward history using 4 points, with and without forced symmetry}
	\label{fig:reward_4_pts_4_pts_boat_tailing}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{\textbf{Best shapes and rewards obtained for boat-tailing with 4 points, with and without forced symmetry.}}
\label{fig:boat_tailing_4pts}
\end{figure} 

==> fig/degenerate_DRL.tex <==
\begin{figure}
\centering
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\myscale{1.0}
\begin{tikzpicture}[	scale=\myscale,
				arrow/.style={thick,color=mybluegray3,rounded corners}]

	%%%%% nodes
	\node[	scale=\myscale,
			rectangle, rounded corners, draw=mygray1, dash pattern=on 2pt, fill=mygray5, ultra thick, 
			text width=16cm, minimum height=2cm, text centered,
			inner sep=0pt, outer sep=0pt] 
			(s) at (6.75,0) {};
	\node[	scale=\myscale] at (14,1.25) {\footnotesize \textbf{1 episode}};
	\node[	scale=\myscale,
			rectangle, rounded corners, draw=mybluegray1, fill=mybluegray4, thick, 
			text width=2cm, minimum height=1cm, text centered,
			inner sep=1pt, outer sep=0pt] 
			(s0) at (0,0) {\footnotesize Initial state};
	\node[	scale=\myscale,
			rectangle, rounded corners, draw=myorange1, fill=myorange4, thick, 
			text width=2cm, minimum height=1cm, text centered,
			inner sep=1pt, outer sep=0pt] 
			(agent) at (4.5,0) {\footnotesize Agent};
	\node[	scale=\myscale,
			rectangle, rounded corners, draw=mygray1, fill=mygray4, thick, 
			text width=2cm, minimum height=1cm, text centered,
			inner sep=1pt, outer sep=0pt] 
			(env) at (9,0) {\footnotesize Environment};
	\node[	scale=\myscale,
			rectangle, rounded corners, draw=myorange1, fill=myorange4, thick, 
			text width=2cm, minimum height=1cm, text centered,
			inner sep=1pt, outer sep=0pt] 
			(agent2) at (13.5,0) {\footnotesize Agent};
	
	%%%%% arrows
	\draw[-stealth,arrow] (s0.east) -- (agent.west);
	\draw[-stealth,arrow] (agent.east) -- (env.west);
	\draw[-stealth,arrow] (env.east) -- (agent2.west);

	%%%%% arrow writings
	\draw[draw=none,postaction={decorate,decoration={raise=0.5ex,text along path,text align=center,text={|\footnotesize|Observation}}}] (s0.east) -- (agent.west);
	\draw[draw=none,postaction={decorate,decoration={raise=0.5ex,text along path,text align=center,text={|\footnotesize|Actions}}}] (agent.east) -- (env.west);
	\draw[draw=none,postaction={decorate,decoration={raise=0.5ex,text along path,text align=center,text={|\footnotesize|Reward}}}] (env.east) -- (agent2.west);

\end{tikzpicture}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{\textbf{Degenerate reinforcement learning framework used in this paper}. One episode consists of a single control from the agent: the same initial observation is provided to the agent at the start, which in return provides an action to the environment. The environment returns a reward value to the agent, and the episode is terminated.}
\label{fig:degenerate_DRL}
\end{figure} 


==> fig/domain.tex <==
\begin{figure}
\centering

\setlength{\fboxsep}{0pt}%
\setlength{\fboxrule}{1pt}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[t]{.45\textwidth}
	\centering
	\fbox{\includegraphics[width=\linewidth]{fig/mesh.png}} 
	\caption{Mesh of the computational domain}
	\label{fig:domain_mesh}
\end{subfigure} \quad
\begin{subfigure}[t]{.45\textwidth}
	\centering
	\fbox{\includegraphics[width=\linewidth]{fig/sol.png}}
	\caption{Computed $v_x$ velocity field at $Re=200$}
	\label{fig:domain_sol}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{\textbf{Mesh and computed $v_x$ velocity field at $Re=100$} behind a random shape. The recirculation area behind the obstacle is clearly visible, followed by a well-established Von Karman vortex alley. The velocity field is scaled in the $\left[-1, 1\right]$ range for displaying purposes.}
\label{fig:domain}
\end{figure} 


==> fig/reward_shaping.tex <==
\begin{figure}
\centering

\setlength{\fboxsep}{0pt}%
\setlength{\fboxrule}{1pt}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[t]{.4\textwidth}
	\centering
	\begin{tikzpicture}[scale=0.875,trim axis left, trim axis right]
		\begin{axis}[	xlabel=lift-to-drag ratio, ylabel=reward, legend pos=north west,
					grid=major,xmin=-10,xmax=10,ymin=-10,ymax=10,legend cell align=left,
					every axis y label/.style={at={(ticklabel cs:0.5)},rotate=90,anchor=near ticklabel}]
			\legend{$r_t$ baseline, $r_t$ shaped}
 
			\addplot[draw=myblue1,ultra thick] 						coordinates {(-10,-5) (-5,-5) (10,10)};
			\addplot[draw=myorange1,ultra thick,dash pattern=on 2pt] 	coordinates {(-10,-5) (-5,-5) (0,0) (5,10)};
		\end{axis}
	\end{tikzpicture}
	\caption{Baseline and shaped reward functions as a function of lift-to-drag ratio}
	\label{fig:reward_functions}
\end{subfigure} \qquad \qquad
\begin{subfigure}[t]{.4\textwidth}
	\centering
	\begin{tikzpicture}[scale=0.875,trim axis left, trim axis right]
		\begin{axis}[	xlabel=episodes, ylabel=reward, legend pos=north west,
					grid=major,xmin=0,xmax=4000,ymin=0,ymax=6,legend cell align=left,
					every axis y label/.style={at={(ticklabel cs:0.5)},rotate=90,anchor=near ticklabel}]
			\legend{$\left<r_t\right>$ baseline, $\left<r_t\right>$ shaped}
 
			\addplot[draw=myblue1,ultra thick,smooth] 	table[x index=0,y index=2] {fig/reward_4_pts_4_pts}; 
			\addplot[draw=myorange1,ultra thick,smooth] 	table[x index=0,y index=2] {fig/reward_4_pts_4_pts_shaped}; 
		\end{axis}
	\end{tikzpicture}
	\caption{Average reward observed during agent learning using baseline and shaped reward functions (normalized)}
	\label{fig:reward_4_pts_4_pts_shaped}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{\textbf{Baseline and shaped reward functions and their resulting observed rewards} on the 4 free points case. Using a shaped reward increases the overall learning speed.}
\label{fig:reward_shaping}
\end{figure} 

==> fig/reward_shaping_area.tex <==
\begin{figure}
\centering

\setlength{\fboxsep}{0pt}%
\setlength{\fboxrule}{1pt}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[t]{.4\textwidth}
	\centering
	\begin{tikzpicture}[scale=0.875,trim axis left, trim axis right]
		\begin{axis}[	xlabel=episodes, ylabel=reward, legend pos=north east,
					grid=major,xmin=0,xmax=4000,ymin=-1,ymax=6,legend cell align=left,
					every axis y label/.style={at={(ticklabel cs:0.5)},rotate=90,anchor=near ticklabel}]
			\legend{$\left<r_t\right>$ baseline, $\left<r_t\right>$ with area constraint}
			
			\addplot[draw=myblue1,ultra thick,smooth] 				table[x index=0,y index=2] {fig/reward_4_pts_3_pts}; 
			\addplot[draw=myorange1,ultra thick,smooth] 				table[x index=0,y index=2] {fig/reward_4_pts_3_pts_area}; 
		\end{axis}
	\end{tikzpicture}
	\caption{Moving-average reward history with and without area constraint}
	\label{fig:reward_area}
\end{subfigure} \qquad \qquad
\begin{subfigure}[t]{.4\textwidth}
	\centering
	\begin{tikzpicture}[scale=0.875,trim axis left, trim axis right]
		\begin{axis}[	xlabel=episodes, ylabel=shape area ($\alpha$), legend pos=north east,
					grid=major,xmin=0,xmax=4000,ymin=2,ymax=4,legend cell align=left,
					every axis y label/.style={at={(ticklabel cs:0.5)},rotate=90,anchor=near ticklabel}]
			\legend{$\alpha$ baseline, $\alpha$ shaped, $\alpha$ target}
			
			\addplot[draw=myblue1,ultra thick,smooth] 				table[x index=0,y index=2] {fig/area_no_constraint}; 
			\addplot[draw=myorange1,ultra thick,smooth] 				table[x index=0,y index=2] {fig/area_constraint_2}; 
			\addplot[draw=mybluegray2,ultra thick,dash pattern=on 2pt]	coordinates {(0,3.14) (4000,3.14)};
		\end{axis}
	\end{tikzpicture}
	\caption{Moving-average area history with and without area constraint}
	\label{fig:area_area}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{\textbf{Moving-average reward and area history of the explored shapes using baseline and shaped reward (\ref{eq:shaped_reward_area}) compared to target area}. Once the learning plateau is reached (approx. 2000 episodes), the agent modifies its behavior in order to fulfill the additional area constraint, although this is barely visible on the reward curve.}
\label{fig:reward_shaping_area}
\end{figure} 

==> fig/shape.tex <==
\begin{figure}
\centering

\setlength{\fboxsep}{0pt}%
\setlength{\fboxrule}{1pt}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fbox{\includegraphics[width=.4\linewidth]{fig/shape.png}} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{\textbf{Example of generated shape with geometrical constraints.} The colored dots indicate the control points generated by the agent, that are then joined using B\'ezier curves. Each point the agent suggests is restricted by construction in radius (inner and outer circles of radii $r_{\text{min}}$ and $r_{\text{max}}$) and in azimuth (diverging white lines).}
\label{fig:shape}
\end{figure} 

==> fig/shape_generation.tex <==
\begin{figure}
\centering
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\xaxis{3}
\def\yaxis{3}
\def\sc{1.0}

\def\pOneX{0.7}
\def\pOneY{0.25}

\def\pTwoX{-0.2}
\def\pTwoY{0.5}

\def\pThreeX{-0.7}
\def\pThreeY{-0.3}

\def\pFourX{0.4}
\def\pFourY{-0.6}

\def\rad{0.5}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Scatter points
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}{.45\textwidth}
	\centering
	\begin{tikzpicture}[	scale=\sc,
					axes/.style={thick,->,-stealth},
					pt/.style={circle,inner sep=0pt,text width=2mm,fill=myblue1,draw=black}]

	%%% Axes 
	\draw[axes] (-\xaxis,0) -- (\xaxis,0) node[anchor=north] {$x$};
	\draw[axes] (0,-\yaxis) -- (0,\yaxis) node[anchor=west] {$y$};

	%%% Nodes
	\node[pt, label=above:$p_1$] 	(p1) at ( \pOneX*\xaxis, 	\pOneY*\yaxis) {};
	\node[pt, label=above:$p_2$] 	(p2) at (\pTwoX*\xaxis, 	\pTwoY*\yaxis) {};
	\node[pt, label=below:$p_3$] 	(p3) at (\pThreeX*\xaxis,	\pThreeY*\yaxis) {};
	\node[pt, label=below:$p_4$] 	(p4) at (\pFourX*\xaxis,	\pFourY*\yaxis) {};

	%%% Increasing angle
	\draw[->,-stealth,dash pattern=on 1pt] (0,0) -- (0.4*\xaxis,0.7*\yaxis);
	\draw[->,-stealth,thick] (0,0) ++(0:1.0) arc (0:60:1.0) node[pos=0.45,xshift=0.15cm,yshift=0.15cm] {$\theta$};

	\end{tikzpicture}
	
	\caption{Sort the provided points by ascending trigonometric angle}
	\label{fig:shape_generation_1}
\end{subfigure} \qquad
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Handle angles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}{.45\textwidth}
	\centering
	\begin{tikzpicture}[	scale=\sc,
					axes/.style={thick,->,-stealth},
					pt/.style={circle,inner sep=0pt,text width=2mm,fill=myblue1,draw=black}]

	%%% Axes 
	\draw[axes] (-\xaxis,0) -- (\xaxis,0) node[anchor=north] {$x$};
	\draw[axes] (0,-\yaxis) -- (0,\yaxis) node[anchor=west] {$y$};

	%%% Nodes
	\node[pt, label=above:$p_1$] 	(p1) at ( \pOneX*\xaxis, 	\pOneY*\yaxis) {};
	\node[pt, label=above:$p_2$] 	(p2) at (\pTwoX*\xaxis, 	\pTwoY*\yaxis) {};
	\node[pt, label=below:$p_3$] 	(p3) at (\pThreeX*\xaxis,	\pThreeY*\yaxis) {};
	\node[pt, label=below:$p_4$] 	(p4) at (\pFourX*\xaxis,	\pFourY*\yaxis) {};
	
	%%% Arrows between nodes
	\draw[->,-stealth,dash pattern=on 1pt] (p1) -- (p2);
	\draw[->,-stealth,dash pattern=on 1pt] (p2) -- (p3);
	
	%%% Angle between p1 and p2
	\draw[dash pattern=on 0.5pt] (\pOneX*\xaxis,\pOneY*\yaxis) -- (\pTwoX*\xaxis,\pOneY*\yaxis);
	\draw[dash pattern=on 0.5pt] (\pTwoX*\xaxis,\pTwoY*\yaxis) -- (\pTwoX*\xaxis,\pOneY*\yaxis);
	\draw[->,-stealth,thick] (\pOneX*\xaxis,\pOneY*\yaxis) ++(164.5:1.25) arc (164.5:180:1.25) node[pos=0.5,xshift=-0.4cm,yshift=0.1cm] {$\theta_{12}$};
	
	%%% Angle between p2 and p3
	\draw[dash pattern=on 0.5pt] (\pTwoX*\xaxis,\pTwoY*\yaxis) -- (\pTwoX*\xaxis,\pThreeY*\yaxis);
	\draw[dash pattern=on 0.5pt] (\pThreeX*\xaxis,\pThreeY*\yaxis) -- (\pTwoX*\xaxis,\pThreeY*\yaxis);
	\draw[->,-stealth,thick] (\pTwoX*\xaxis,\pTwoY*\yaxis) ++(238:1.0) arc (238:270:1.0) node[pos=0.5,xshift=-0.1cm,yshift=-0.3cm] {$\theta_{23}$};
	
	%%% Redraw nodes
	\node[pt, label=above:$p_1$] 	(p1) at ( \pOneX*\xaxis, 	\pOneY*\yaxis) {};
	\node[pt, label=above:$p_2$] 	(p2) at (\pTwoX*\xaxis, 	\pTwoY*\yaxis) {};
	\node[pt, label=below:$p_3$] 	(p3) at (\pThreeX*\xaxis,	\pThreeY*\yaxis) {};
	\node[pt, label=below:$p_4$] 	(p4) at (\pFourX*\xaxis,	\pFourY*\yaxis) {};

	\end{tikzpicture}
	
	\caption{Compute angles between points, and compute an average angle around each point $\theta^*_i$}
	\label{fig:shape_generation_2}
\end{subfigure}%

\medskip
\medskip
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Draw cubic Bezier curve
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}{.45\textwidth}
	\centering
	\begin{tikzpicture}[	scale=\sc,
					axes/.style={thick,->,-stealth},
					pt/.style={circle,inner sep=0pt,text width=2mm,fill=myblue1,draw=black}]

	%%% Axes 
	\draw[axes] (-\xaxis,0) -- (\xaxis,0) node[anchor=north] {$x$};
	\draw[axes] (0,-\yaxis) -- (0,\yaxis) node[anchor=west] {$y$};

	%%% Nodes
	\node[pt, label=above:$p_1$] 	(p1) at ( \pOneX*\xaxis, 	\pOneY*\yaxis) {};
	\node[pt, label=above:$p_2$] 	(p2) at (\pTwoX*\xaxis, 	\pTwoY*\yaxis) {};
	\node[pt, label=below:$p_3$] 	(p3) at (\pThreeX*\xaxis,	\pThreeY*\yaxis) {};
	\node[pt, label=below:$p_4$] 	(p4) at (\pFourX*\xaxis,	\pFourY*\yaxis) {};
	
	%%% Bezier nodes
	\node[pt, label=left:$p^*_2$] 	(p2s) at (\pTwoX*\xaxis-0.989*\rad*\xaxis, \pTwoY*\yaxis-0.147*\rad*\yaxis) {};
	\node[pt, label=left:$p^{**}_2$] 	(p2ss) at (\pThreeX*\xaxis-0.147*\rad*\xaxis, \pThreeY*\yaxis+0.989*\rad*\yaxis) {};
	
	%%% Arrows between nodes
	\draw[->,-stealth,dash pattern=on 1pt] (p1) -- (p2);
	\draw[->,-stealth,dash pattern=on 1pt] (p2) -- (p3);
	
	%%% Additional lines to draw and average angle
	\draw[dash pattern=on 0.5pt] (p2) -- (p2s);
	\draw[dash pattern=on 0.5pt] (p3) -- (p2ss);
	\node[draw=none] (p2t) at (\pTwoX*\xaxis-0.963*\rad*\xaxis, \pTwoY*\yaxis+0.267*\rad*\yaxis) {};
	\draw[dash pattern=on 1pt] (p2) -- (p2t);
	\draw[->,-stealth,thick] (\pTwoX*\xaxis,\pTwoY*\yaxis) ++(164.5:0.8) arc (164.5:188:0.8) node[pos=0.5,xshift=-0.35cm,yshift=0.03cm] {$\theta^*_2$};
	
	%%% Cubic Bezier curve
	\draw[thick,myorange1] (p2) .. controls (p2s) and (p2ss) .. (p3);
	
	%%% Redraw nodes
	\node[pt, label=above:$p_1$] 	(p1) at ( \pOneX*\xaxis, 	\pOneY*\yaxis) {};
	\node[pt, label=above:$p_2$] 	(p2) at (\pTwoX*\xaxis, 	\pTwoY*\yaxis) {};
	\node[pt, label=below:$p_3$] 	(p3) at (\pThreeX*\xaxis,	\pThreeY*\yaxis) {};
	\node[pt, label=below:$p_4$] 	(p4) at (\pFourX*\xaxis,	\pFourY*\yaxis) {};

	\end{tikzpicture}
	
	\caption{Compute control points coordinates from averaged angles and generate cubic B\'ezier curve}
	\label{fig:shape_generation_3}
\end{subfigure} \qquad
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Draw cubic Bezier curve
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}{.45\textwidth}
	\centering
	\begin{tikzpicture}[	scale=\sc,
					axes/.style={thick,->,-stealth},
					pt/.style={circle,inner sep=0pt,text width=2mm,fill=myblue1,draw=black},
					sample/.style={circle,inner sep=0pt,text width=1mm,fill=mygray1,draw=black}]

	%%% Axes 
	\draw[axes] (-\xaxis,0) -- (\xaxis,0) node[anchor=north] {$x$};
	\draw[axes] (0,-\yaxis) -- (0,\yaxis) node[anchor=west] {$y$};

	%%% Nodes
	\node[pt, label=above:$p_1$] 	(p1) at ( \pOneX*\xaxis, 	\pOneY*\yaxis) {};
	\node[pt, label=above:$p_2$] 	(p2) at (\pTwoX*\xaxis, 	\pTwoY*\yaxis) {};
	\node[pt, label=below:$p_3$] 	(p3) at (\pThreeX*\xaxis,	\pThreeY*\yaxis) {};
	\node[pt, label=below:$p_4$] 	(p4) at (\pFourX*\xaxis,	\pFourY*\yaxis) {};
	
	%%% Bezier nodes
	\node[draw=none] 	(p2s) at (\pTwoX*\xaxis-0.989*\rad*\xaxis, \pTwoY*\yaxis-0.147*\rad*\yaxis) {};
	\node[draw=none] 	(p2ss) at (\pThreeX*\xaxis-0.147*\rad*\xaxis, \pThreeY*\yaxis+0.989*\rad*\yaxis) {};
	\node[draw=none] 	(p3s) at (\pThreeX*\xaxis+0.147*\rad*\xaxis, \pThreeY*\yaxis-0.989*\rad*\yaxis) {};
	\node[draw=none] 	(p3ss) at (\pFourX*\xaxis-0.6*\rad*\xaxis, \pFourY*\yaxis-0.5*\rad*\yaxis) {};
	\node[draw=none] 	(p4s) at (\pFourX*\xaxis+0.6*\rad*\xaxis, \pFourY*\yaxis+0.5*\rad*\yaxis) {};
	\node[draw=none] 	(p4ss) at (\pOneX*\xaxis+0.4*\rad*\xaxis, \pOneY*\yaxis-0.5*\rad*\yaxis) {};
	\node[draw=none] 	(p1s) at (\pOneX*\xaxis-0.4*\rad*\xaxis, \pOneY*\yaxis+0.5*\rad*\yaxis) {};
	\node[draw=none] 	(p1ss) at (\pTwoX*\xaxis+0.989*\rad*\xaxis, \pTwoY*\yaxis+0.147*\rad*\yaxis) {};
	
	%%% Cubic Bezier curve
	\draw[thick,myorange1] (p2) .. controls (p2s) and (p2ss) .. (p3);
	\draw[thick,myorange1] (p3) .. controls (p3s) and (p3ss) .. (p4);
	\draw[thick,myorange1] (p4) .. controls (p4s) and (p4ss) .. (p1);
	\draw[thick,myorange1] (p1) .. controls (p1s) and (p1ss) .. (p2);
	
	%%% Samples on Bezier curve
	\draw[draw=none] (p4) .. controls (p4s) and (p4ss) .. (p1) node[sample,pos=0.1,opacity=1] {};
	\draw[draw=none] (p4) .. controls (p4s) and (p4ss) .. (p1) node[sample,pos=0.2,opacity=1] {};
	\draw[draw=none] (p4) .. controls (p4s) and (p4ss) .. (p1) node[sample,pos=0.3,opacity=1] {};
	\draw[draw=none] (p4) .. controls (p4s) and (p4ss) .. (p1) node[sample,pos=0.4,opacity=1] {};
	\draw[draw=none] (p4) .. controls (p4s) and (p4ss) .. (p1) node[sample,pos=0.5,opacity=1] {};
	\draw[draw=none] (p4) .. controls (p4s) and (p4ss) .. (p1) node[sample,pos=0.6,opacity=1] {};
	\draw[draw=none] (p4) .. controls (p4s) and (p4ss) .. (p1) node[sample,pos=0.7,opacity=1] {};
	\draw[draw=none] (p4) .. controls (p4s) and (p4ss) .. (p1) node[sample,pos=0.8,opacity=1] {};
	\draw[draw=none] (p4) .. controls (p4s) and (p4ss) .. (p1) node[sample,pos=0.9,opacity=1] {};
	
	%%% Redraw nodes
	\node[pt, label=above:$p_1$] 	(p1) at ( \pOneX*\xaxis, 	\pOneY*\yaxis) {};
	\node[pt, label=above:$p_2$] 	(p2) at (\pTwoX*\xaxis, 	\pTwoY*\yaxis) {};
	\node[pt, label=below:$p_3$] 	(p3) at (\pThreeX*\xaxis,	\pThreeY*\yaxis) {};
	\node[pt, label=below:$p_4$] 	(p4) at (\pFourX*\xaxis,	\pFourY*\yaxis) {};

	\end{tikzpicture}
	
	\caption{Sample all B\'ezier lines and export for mesh immersion}
	\label{fig:shape_generation_4}
\end{subfigure}% \qquad \qquad
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{\textbf{Shape generation using cubic B\'ezier curves}. Each subfigure illustrates one of the consecutive steps used in the process. Detailed nomenclature is provided in the text.}
\label{fig:shape_generation}
\end{figure} 

==> fig/wing_4pts.tex <==
\begin{figure}
\centering

\setlength{\fboxsep}{0pt}%
\setlength{\fboxrule}{1pt}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[t]{.25\textwidth}
	\centering
	\fbox{\includegraphics[width=\linewidth]{fig/4_pts_1_pt.png}} 
	\caption{Best shape with 4 points, 1 free point (3 d.o.f.s)}
	\label{fig:4_pts_1_pt}
\end{subfigure} \qquad
\begin{subfigure}[t]{.25\textwidth}
	\centering
	\fbox{\includegraphics[width=\linewidth]{fig/4_pts_3_pts.png}} 
	\caption{Best shape with 4 points, 3 free points (9 d.o.f.s)}
	\label{fig:4_pts_3_pts}
\end{subfigure} \qquad
\begin{subfigure}[t]{.25\textwidth}
	\centering
	\fbox{\includegraphics[width=\linewidth]{fig/4_pts_4_pts.png}} 
	\caption{Best shape with 4 points, 4 free points (12 d.o.f.s)}
	\label{fig:4_pts_4_pts}
\end{subfigure}

\bigskip

\begin{subfigure}[t]{.85\textwidth}
	\centering
	\fbox{\includegraphics[width=\linewidth]{fig/4_pts_4_pts_sol.png}} 
	\caption{Computed $v_x$ velocity field at $Re \sim 600$ around shape \ref{fig:4_pts_4_pts} (the domain is cropped).}
	\label{fig:4_pts_4_pts_u}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{\textbf{Results of the shape optimization process}. Best shapes obtained using 1, 3 and 4 free points are shown in subfigures \ref{fig:4_pts_1_pt}, \ref{fig:4_pts_3_pts} and \ref{fig:4_pts_4_pts} respectively. In subfigure \ref{fig:4_pts_1_pt}, the left, top and bottom points are fixed to their initial position (\ie that of the reference cylinder) while the rightmost one is free to move. In subfigure \ref{fig:4_pts_3_pts}, only the left point is fixed, while in subfigure \ref{fig:4_pts_4_pts}, all four points are free to move. The velocity field corresponding to shape \ref{fig:4_pts_4_pts} is shown in subfigure \ref{fig:4_pts_4_pts_u}.}
\label{fig:wing_4pts}
\end{figure} 

==> fig/wing_4pts_reward.tex <==
\begin{figure}
\centering

\setlength{\fboxsep}{0pt}%
\setlength{\fboxrule}{1pt}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}[t]{.4\textwidth}
	\centering
	\begin{tikzpicture}[scale=0.875,trim axis left, trim axis right]
		\begin{axis}[	xlabel=episodes, ylabel=reward,
					grid=major,xmin=0,xmax=4000,ymin=-2,ymax=8,legend cell align=left,
            				every axis y label/.style={at={(ticklabel cs:0.5)},rotate=90,anchor=near ticklabel}]
			\legend{\,\,$r_t$,$\left<r_t\right>$}
 
			\addplot[draw=myblue2,thick,smooth] 		table[x index=0,y index=1] {fig/reward_4_pts_4_pts}; 
			\addplot[draw=myorange1,ultra thick,smooth] 	table[x index=0,y index=2] {fig/reward_4_pts_4_pts}; 
		\end{axis}
	\end{tikzpicture}	
	\caption{Instantaneous and moving-average reward history using 4 free points}
	\label{fig:reward_4_pts_4_pts}
\end{subfigure} \qquad \qquad
\begin{subfigure}[t]{.4\textwidth}
	\centering
	\begin{tikzpicture}[scale=0.875,trim axis left, trim axis right]
		\begin{axis}[	xlabel=episodes, ylabel=reward, legend pos=north west,
					grid=major,xmin=0,xmax=4000,ymin=0,ymax=6,legend cell align=left,
            				every axis y label/.style={at={(ticklabel cs:0.5)},rotate=90,anchor=near ticklabel}]
			\legend{$\left<r_t\right>$ 1 pt., $\left<r_t\right>$ 3 pts., $\left<r_t\right>$ 4 pts.}
 
			\addplot[draw=myblue1,ultra thick,smooth] 	table[x index=0,y index=2] {fig/reward_4_pts_1_pt}; 
			\addplot[draw=mybluegray1,ultra thick,smooth] 	table[x index=0,y index=2] {fig/reward_4_pts_3_pts}; 
			\addplot[draw=myorange1,ultra thick,smooth] 	table[x index=0,y index=2] {fig/reward_4_pts_4_pts}; 
		\end{axis}
	\end{tikzpicture}	
	\caption{Moving-average reward history using 1, 3 and 4 free points}
	\label{fig:reward_averaged}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption{\textbf{Typical reward evolution (instantaneous and averaged)} during the shape optimization process. Subfigure \ref{fig:reward_4_pts_4_pts} corresponds to the learning of shape \ref{fig:4_pts_4_pts}. Averaged learning curves for the three different cases of figure \ref{fig:wing_4pts} are compared in subfigure \ref{fig:reward_averaged}.}
\label{fig:wing_4pts_reward}
\end{figure} 
